The Pay and Non-Pay Content of Job Ads

How informative are job ads about the actual pay and non-pay attributes offered by employers? Using a comprehensive database of job ads posted by Norwegian employers, we develop a methodology to systematically classify the pay and non-pay job attributes advertised in vacancy texts. About 60% of job ads provide pay-related information and nearly all ads feature information on non-pay attributes. We link these advertised attributes to the employers posting the ads and validate this information against revealed-preference measures of employer quality, realized attributes, and choices from a survey experiment. All three strategies confirm that job ads provide reliable signals of employer quality. We then incorporate the detailed job attributes in a monopsony framework and quantify their contribution to labor market inequality.

==> tables/sample_selection/balance_2015_2024.tex <==
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{lccccc} \hline\midrule
 & & \multicolumn{2}{c}{\textbf{Main Analysis}} & \multicolumn{2}{c}{\textbf{Addititional Analysis}} \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6}
&\shortstack{All\\Observations}&\shortstack{Text\\Analysis\\Sample}&\shortstack{Employer\\Quality\\Sample}&\shortstack{Linked\\Ad-Hire\\Sample}&\shortstack{Survey\\Experiment\\Sample}  \\ 
& \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)} & \multicolumn{1}{c}{(4)} & \multicolumn{1}{c}{(5)} \\ 
\midrule 
\textbf{Worker Characteristics:} & & & & & \\
\quad Age &41.9 &41.6 &40.0 &42.1 &42.5 \\
\quad Immigrant &15.6\% &15.6\% &16.6\% &14.4\% &17.6\% \\
\quad Women &46.5\% &47.3\% &49.4\% &51.2\% &54.7\% \\
\quad College &50.0\% &50.6\% &53.4\% &54.2\% &62.9\% \\
\quad Hourly Wage &\$29.75 &\$29.79 &\$30.49 &\$30.15 &\$31.06 \\
\quad Number of Workers &3,479,076 &3,383,123 &2,956,702 &2,839,495 &462,185 \\
\quad Number of Worker-Years &29,789,720 &28,328,064 &23,470,708 &20,005,948 &2,067,996 \\
\textbf{Establishment Characteristics:} & & & & & \\
\quad Size &14.6 &20.6 &22.6 &32.7 &61.1 \\
\quad Public Sector &14.0\% &19.2\% &20.3\% &27.6\% &45.6\% \\
\quad Industry Composition & & & & & \\
\quad\quad Agriculture, Forestry and Fishing &3.0\% &1.9\% &1.5\% &0.9\% &0.2\% \\
\quad\quad Mining and Quarrying &0.4\% &0.4\% &0.4\% &0.3\% &0.0\% \\
\quad\quad Manufacturing &4.7\% &5.1\% &4.9\% &5.4\% &1.5\% \\
\quad\quad Energy Supply &0.4\% &0.4\% &0.4\% &0.5\% &0.5\% \\
\quad\quad Water Supply &0.5\% &0.6\% &0.6\% &0.6\% &1.2\% \\
\quad\quad Construction &12.5\% &10.6\% &10.1\% &7.5\% &5.1\% \\
\quad\quad Wholesale and Retail Trade &20.0\% &23.0\% &23.7\% &25.9\% &19.6\% \\
\quad\quad Transportation and Storage &5.1\% &4.9\% &5.0\% &3.4\% &8.1\% \\
\quad\quad Accommodation and Food Service &5.0\% &6.2\% &6.0\% &4.7\% &7.5\% \\
\quad\quad Information and Communication &3.9\% &3.3\% &3.7\% &2.5\% &1.7\% \\
\quad\quad Financial and Insurance &1.1\% &1.1\% &1.1\% &1.2\% &0.9\% \\
\quad\quad Real Estate &4.2\% &2.2\% &1.9\% &1.4\% &0.4\% \\
\quad\quad Professional, Scientific and Technical &9.7\% &7.1\% &7.3\% &5.6\% &3.5\% \\
\quad\quad Administrative and Support Service &4.5\% &4.5\% &3.5\% &3.0\% &9.0\% \\
\quad\quad Public Administration and Defence &2.1\% &2.9\% &2.8\% &4.0\% &6.2\% \\
\quad\quad Education &3.3\% &4.1\% &4.5\% &6.3\% &5.2\% \\
\quad\quad Health and Social Work &12.4\% &14.9\% &16.4\% &21.3\% &24.8\% \\
\quad\quad Arts, Entertainment and Recreation &2.6\% &2.6\% &2.4\% &1.9\% &1.1\% \\
\quad\quad Other Service Activities &4.4\% &4.1\% &3.7\% &3.6\% &3.6\% \\
\quad\quad Households as Employers &0.1\% &0.0\% &0.0\% &0.0\% &0.0\% \\
\quad\quad Extraterritorial Organisations and Nodies &0.0\% &0.0\% &0.0\% &0.0\% &0.0\% \\
\quad Number of Establishments &359,790 &196,231 &162,346 &71,866 &538 \\
\midrule\hline
\end{tabular}


==> tables/vacancy_duration/vacancy_duration_c_nc_2015_2024.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
                    &\multicolumn{2}{c}{Outcome: Log Vacancy Duration}                                                           \\
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
\hline
\multicolumn{3}{l}{\textbf{Separate Regressions:}} \\

Posted Pay Premium  &       -0.014\sym{**}&  0.080\sym{***}   \\
                    &     (0.007)         &  (0.016)          \\
[1em]
Posted Overall Sorkin Value&-0.020\sym{***}  &     -0.089\sym{***} \\
                    &  (0.006)            &     (0.026) \\
[1em]
Posted Poaching Index&  -0.024\sym{***}  &   -0.051\sym{***}  \\
                    &   (0.005)          &   (0.023)     \\
[1em]
Occupation FE       &         &  \checkmark   \\
[1em]
Industry FE         &          &  \checkmark   \\
[1em]
Location FE        &           &  \checkmark  \\
\hline
Employer Clusters   &       3,271      &   3,271    \\
Establishments      &      162,346    &    162,346   \\
Ads                 &    1,998,745      &   1,998,745   \\
Worker-Years        &    28,328,064      &  28,328,064    \\
\hline\hline
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}

